Hybrid Paul-optical trap with large optical access for levitated optomechanics

We present a hybrid trapping platform that allows us to levitate a charged nanoparticle in high vacuum using either optical fields, radio-frequency fields, or a combination thereof. Our hybrid approach combines an optical dipole trap with a linear Paul trap while maintaining a large numerical aperture (0.77 NA). We detail a controlled transfer procedure that allows us to use the Paul trap as a safety net to recover particles lost from the optical trap at high vacuum. The presented hybrid platform adds to the toolbox of levitodynamics and represents an important step towards fully controllable dark potentials, providing control in the absence of decoherence due to photon recoil.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
